SHARC: Reference point driven Spherical Harmonic Representation for Complex Shapes

We propose SHARC, a novel framework that synthesizes arbitrary, genus-agnostic shapes by means of a collection of Spherical Harmonic (SH) representations of distance fields. These distance fields are anchored at optimally placed reference points in the interior volume of the surface in a way that maximizes learning of the finer details of the surface. To achieve this, we employ a cost function that jointly maximizes sparsity and centrality in terms of positioning, as well as visibility of the surface from their location. For each selected reference point, we sample the visible distance field to the surface geometry via ray-casting and compute the SH coefficients using the Fast Spherical Harmonic Transform (FSHT). To enhance geometric fidelity, we apply a configurable low-pass filter to the coefficients and refine the output using a local consistency constraint based on proximity. Evaluation of SHARC against state-of-the-art methods demonstrates that the proposed method outperforms existing approaches in both reconstruction accuracy and time efficiency without sacrificing model parsimony. The source code is available at https://github.com/POSE-Lab/SHARC.

==> sections/Introduction.tex <==
Representing complex 3D geometry in a way that is both compact and structurally expressive remains a central challenge in computer graphics, geometry processing, and 3D generative modeling. Explicit representations, such as triangle meshes and dense point clouds, serve as industry standards but often suffer from high dimensionality, and irregularity, making them expensive to transmit, edit, or utilize in optimization tasks. On the other hand, implicit neural fields encode shapes in the weights of deep networks or low-dimensional latent codes, enabling high-quality reconstruction and generative modeling. Yet, these advantages come at the cost of an opaque internal structure lacking interpretability and a non-trivial decoding expense \cite{Chen2019,Zhang2023_3dshape2vecset}. Consequently, despite their generative capabilities, the high evaluation cost and parameter overhead make them less attractive as final, storable geometry codes. These limitations become particularly acute is settings like large-scale 3D repositories, interactive or embedded systems, and text-to-3D pipelines, where the balance between bitrate efficiency and structural control is paramount. There is a growing need for alternative 3D encodings that retain the analytical clarity of classical geometric primitives, approach or surpass the compression of neural codecs, and integrate naturally with learning-based pipelines.

Medial and skeletal representations address part of this problem by providing a lower-dimensional structural scaffold for shapes. Extensive work in this field has shown that unions of spheres or generalized medial primitives can approximate solids and surfaces with controlled error \cite{bradshaw2004,Foskey2003,Giesen2009scale_transform,Miklos2010,Sun2016medial_mesh}. % Methods such as \cite{stolpner2012_medial_spheres,Sun2016medial_mesh} approximate volumes using spheres and convex hulls of small sphere sets, with simplification guided by Hausdorff distance to the input. 
Subsequent formulations treat skeletal extraction as a coverage or optimization problem \cite{dou2022coverage,wang2024coverage,Rebain2019_lsmat} and related greedy schemes prioritizing large, structurally meaningful balls under geometric constraints \cite{Dou2021}. More recent work \cite{Guo2023MSD,Wang2022,Wang2024_mattopo} augments these ideas with structural and topological guarantees using restricted power diagrams, producing high-quality medial meshes. The community has also begun to exploit medial structure as a learnable representation where unsupervised or weakly supervised methods infer skeletons or medial meshes directly from point clouds \cite{Ge2023_point2mm,Lin2021_point2skeleton,Yang2020_P2MAT-Net}.

At the same time, learning-based methods have made major strides in compact 3D generative modeling. While implicit decoders \cite{Zhang2023_3dshape2vecset,Chen2019} achieve impressive quality, their shape codes remain unintelligible. Complementary approaches explicitly incorparate analystic primitcies \cite{Paschalidou2019} approximating shapes with volumetric pasts, while spherical SDFs \cite{Li2022} exploit spherical domains for efficient compression. Other approaches \cite{petrov2024gem3d} utilize media-axis skeletons for topology-aware generation. 

Spherical Harmonics (SH) and spectral representations offer a complementary avenue for compact encoding. While global fitting schemes \cite{shen2006sh,Li2024FSH3D} effectively encode genus-zero geometry, handling arbitrary topology often requires decomposing shapes into local spherical patches via spatial partitioning strategies like kd-trees \cite{mousa2007sh}. More recent approaches \cite{Li-2025-MASH} employ masked SH fields around view-based anchors. Yet, these approaches rely on either global parameterization or spatial partitioning schemes that ignore the shape's natural structure.Consequently, they lack the explicit connection between spectral detail and volumetric topology inherent to medial representations.

Despite these advances, a unified solution remains elusive. Spectral and partitioning schemes often ignore natural articulation, neural fields suffer from opacity and high decoding costs, and standard skeletons lack fine surface detail. Consequently, none of these methods provides a representation that is at once (i) topology-aware and coverage-optimized in the sense of MAT-based skeletons, (ii) endowed with a compact, analytically smooth local field encoding fine detail, and (iii) directly decodable without a heavyweight neural network.

In this work we introduce SHARC, a new 3D shape representation that tightly couples medial skeletal structure with local spherical-harmonic distance fields. SHARC represents a shape by a sparse set of skeletal anchors optimally selected via a visibility-aware coverage score scheme. For each anchor, we encode a sampled distance field through spherical harmonic coefficients. In contrast to classical MAT encodings, SHARC uses the skeleton not only as a coarse volumetric scaffold but also as the coordinate system for high-frequency geometric detail and in contrast to existing SH-bases encodings, the anchors are explicitly tied to the medial geometry and topology of the shape.

The main contributions of this paper include:
\begin{itemize}
    \item A novel Hybrid Shape Representation that integrates skeletal structures with local Spherical Harmonic (SH) fields, effectively bridging the gap between topology-aware medial representations and spectral encoding.
    \item A Visibility-Aware Anchor Selection process building upon \cite{wang2024coverage} that identifies the optimal set of skeletal anchors based on visibility and proximity rather than just volumetric coverage.
    \item A comprehensive pipeline for sampling and learning local radial distance fields using the Fast Spherical Harmonic Transform (FSHT). This facilitates high-fidelity surface reconstruction capable of preserving intricate details in a multi-resolution manner.
    \item Demonstrated versatility across downstream tasks, showcasing that our representation can be efficiently and seamlessly integrated into frameworks for shape compression, text-to-3D generation, and animation.
\end{itemize}
